DISCERN: Designing Decision Support Interfaces to Investigate the Complexities of Workplace Social Decision-Making With Line Managers

Line managers form the first level of management in organizations, and must make complex decisions, while maintaining relationships with those impacted by their decisions. Amidst growing interest in technology-supported decision-making at work, their needs remain understudied. Further, most existing design knowledge for supporting social decision-making comes from domains where decision-makers are more socially detached from those they decide for. We conducted iterative design research with line managers within a technology organization, investigating decision-making practices, and opportunities for technological support. Through formative research, development of a decision-representation tool -- DISCERN -- and user enactments, we identify their communication and analysis needs that lack adequate support. We found they preferred tools for externalizing reasoning rather than tools that replace interpersonal interactions, and they wanted tools to support a range of intuitive and calculative decision-making. We discuss how design of social decision-making supports, especially in the workplace, can more explicitly support highly interactional social decision-making.

==> sections-old/01_introduction_v1.tex <==
% % Relevant Papers:

% % Multiple representations for ideas: https://arxiv.org/pdf/2308.03921.pdf

% % Multi-resolution representations for ideas:
% % https://arxiv.org/pdf/2306.09328.pdf

% % but focuses more on version control

% % Maybe: https://arxiv.org/pdf/2302.14165.pdf

% % Paul Resnick's paper on soliciting expert recommendations can help set up the problem:https://pubsonline.informs.org/doi/abs/10.1287/mnsc.1050.0379


% % Dourish paper ofcourse

% % Decision Analysis for Healthcare Managers (especially the MAV chapter)

% % Decision Synthesis

% In any 

% There is a great disconnect between the design of portable interactive electronics and the design of the energy storage systems
% that power them. Consider the following: Alice is a designer who
% wishes to create a small interactive electronic ring to wear for a
% few hours at an upcoming special event. She begins by prototyping on a benchtop, using a power supply to power her electronics
% and focusing on refning her desired interactions and aesthetic elements, which she can iteratively prototype quickly. Once satisfed,
% Alice makes the appropriate electrical measurements to estimate
% the power consumption of her system. The system turns out to be
% very low power, requiring only 1V and consuming at most 1mA.
% Looking through an online catalogue, Alice fnds that the smallest battery that can suit her needs is a 3.7V, 110mAh lithium ion
% battery that costs \$6 (USD) 1. It will arrive in 2-5 days. While the
% battery is relatively small – half the size of a thumb – it is still large
% for Alice’s on-fnger application and will power the system almost
% 100 times longer than necessary. Alice is further disappointed to
% realize that after the event, she will have no use for the battery,
% and it will simply sit in her drawer and gather dust alongside her
% growing collection of old batteries. While waiting for the battery
% to arrive, Alice adjusts her design, increasing its size substantially
% to accommodate, hide, and protect the battery.

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{images/discern-intro.pdf}
    \caption{}
    TODO update participant count, mentor count, add the fourth incubator, Add one feature during fourth incubator to be "Improved feedback visibility, Add interview w/ 1 entrepreneur in April 2023" 
    \label{fig:timeline}
\end{figure} 



The computer-mediated nature of modern work creates the possibility of collecting and analyzing rich data or `evidence'---both quantitative and qualitative---on which decision-makers may base organizational decisions. Consider the case of a healthcare program manager deciding whether the hospital's budget for quality improvement projects is better spent pursuing improvements in the cardiac care unit or the respiratory care unit. Historical data such as each unit's readmission rates, complication rates, utilization rates, operating costs, or results of routine burnout measurement surveys can inform an assessment of how each potential course of action is anticipated to fare along different criteria. With this orientation, HCI research has featured a number of attempts to help decision-makers make sense of available information in the hopes that this results in decisions that realize better outcomes or at least contributes decision-making processes that are more consistent, efficient, and defensible. 

However, even when using data to make workplace decisions, decision makers must still draw on the experiences of multiple individuals. Making a decision is more than just assessing each option along different criteria. To pick the most attractive option, decision-makers must first make value judgments about what objective the decision ought to accomplish---which criteria should even be considered and the relative value placed on each. Because organizational decisions involve shared costs and responsibilities, defining the importance of different criteria requires a decision-maker to consider the perspectives of, or at least seek acceptance from, multiple stakeholders. In the above example, for instance, hospital administrators might care most about reducing operating costs whereas healthcare providers might care most about reducing readmissions. What would characterize a `better' investment? Further, a decision-maker might also learn from stakeholders with relevant expertise how the achievement of certain objectives ought to be measured, whether through existing data or otherwise. For instance, healthcare providers might specifically want to reduce readmissions that result from inadequate follow-up and medication errors as opposed to all readmissions. Finally, when there is inadequate data or when the problem representation does not warrant precise data-based assessment, decision-makers may advance by soliciting the individual opinion of relevant stakeholders (unit leaders might help judge perceived levels of burnout or fatigue in each unit when available data from surveys is prone to under-reporting). Thus, in advance of or in parallel to any attempt to make decisions in the presence of data, decision-makers also engage in a value-focused deliberative process that engages relevant stakeholders. If collecting and analyzing data provides the means to "optimizing", the adjacent deliberative process represents the process of designing the optimization problem itself: recognizing and representing the objectives and the constraints.

Unfortunately, we still lack representational structures that can effectively support the deliberation adjacent to organizational decisions. We encountered this issue through our formative work focused on studying how managers within a large multinational tech company gathered, organized, and analyzed evidence relevant to workplace decisions but we are hardly the first to suggest this. Managers believed the scarce resource was not `evidence' and the means to analyze it but good representations to capture and externalize the messy and iterative deliberative process. We found that the process of incorporating values of different stakeholders into decision-making criteria and trade-offs, reasoning about how criteria should be measured, and collecting judgements to arriving at a final decision was iterative and spanned disjointed information sources as well as written and verbal discourse. To help with the process, managers often used techniques such as building comparison tables using spreadsheets or notepads. But while these provided a convenient way to immediately capture relevant data in one place, they were reported to be a poor representation for the reflective and iterative reasoning about values. Keeping track of how judgements were made and criteria were weighed was challenging because appropriate representations were thought not to exist or lived outside the context. 

This paper focuses on the deliberation inherent in many organizational decisions, asking if (and how) intelligent tools can support it. In doing so, we report on a series of design activities conducted with managers in a large tech company, reflecting on our activities, designed artifacts, how managers responded to our design choices, and the design opportunities they (and we) identified. Through formative surveys and interviews we examined managers' current practices of deliberative reasoning reflecting on what intelligent tools might support. Based on our findings, we developed \textbf{DISCERN}, an Excel extension. Finally, we conducted user enactments, asking four managers to enact a loosely scripted scenario they were familiar with---a simulation of a team meeting in which they are attempting to make decision---with and without our design concept---DISCERN. We used these enactments as boundary objects inviting managers to reflect on how DISCERN supported or complicated their needs, to observe underlying social boundaries, and to further identify opportunities for possible system designs.

Through this process we found that ....










% There is growing interest in understanding how individuals tasked with making institutional decisions can leverage this data to make `better' decisions conceived as either realizing `better' outcomes than otherwise possible or as a more efficient, consistent, and justifiable decison-making process.



% When tasked with making decisions for a collective, how might information tools help a decision-maker assess the costs and benefits of different courses of action when the very judgement of what is characterized as a `cost' and a `benefit' as well as judgements of their severity must consider the perspectives of, or atleast seek acceptance from, the collective? At their core, many decisions involve an assessment---whether formal or informal---of costs and benefits (or pros and cons) corresponding to different courses of action to pick the option that is anticipated to be the most attractive overall. Within HCI research, a common perspective is that historical data can help people make `better' decisions because it can help them apply their own and others' experiences towards making better judgements about costs and benefits. With this orientation, there has been significant interest in developing tools to support personal decision-making that help individuals make sense of historical data (e.g online reviews) to refine their judgements about the severity of costs and benefits associated with different courses of action and the likelihood of realizing them. Alongside, several attempts have been made to extend this approach to develop information processing tools and interfaces to help institutional decision-makers collect, explore, and analyze the high-resolution data generated by information work to make decisions that are `better'---conceived as either realizing better outcomes than would have been otherwise possible, or a more efficient, consistent and justifiable decision-making process. However, unlike decisions made by an individual for themselves, decisions that result in shared costs and responsibilities require decision-makers to consider the preferences and perspectives of different stakeholders in advance of or in parallel to decision-making to assess the costs, benefits, and overall attractiveness of choice alternatives. Of course decisions can be made by those with authority even without such considerations but those decisions may fail to be enforced if they do not enjoy collective buy-in.

% Unfortunately, the process through which decision-makers attempt to socially negotiate evaluations of costs and benefits is often iterative and can generate information that is hard to structure and manage in a way that supports effective reasoning about, and communicating, cost and benefits. Our formative work


% In many institutional decisions---decisions involving shared costs and responsibilities---decision-makers must consider what different stakeholders \textit{value} when assessing the attractiveness of potential outcomes corresponding to different choice alternatives. Most theories of decision-making suggest that a decision-maker assesses the attractiveness and likelihood of the possible outcomes of choice alternatives, albeit subjectively and possibly with bias or error, and integrates this information through some type of expectation-based calculus to arrive at a decision. The process is admittedly subjective because the decision-maker's values---what they intrinsically deem important or desirable--- determine the attractiveness of outcomes, forming the basis for an evaluative conclusion.  



% In many decisions, however, the way in which `desirability' is defined and evaluated is itself conclusive.





% Consider the following: Alice is a healthcare program manager attempting to decide whether the hospital's budget for quality improvement projects is `better' spent pursuing improvements in the trauma unit or the stroke unit. Each alternative has merits but limited resources require that only one be chosen. Improvements to the stroke unit are judged to be more congruent with the hospital's strategic plans as well as the immediate demands of the staff however forecasts suggest that improvements to the trauma unit would help the hospital better cope with rising patient care demands. If the hospital's forecasted ability to 


% Although this is a hypothetical scenario, many organizational decisions

% Most theories of decision-making suggest that people make decisions by assessing the consequences of potential choice alternatives and committing to the alternative that leads to the most desirable consequences. But how are consequences corresponding to some choice alternatives judged to be `good' or `better' and those corresponding to other alternatives judged `bad' or `worse'  When modeling decisions, it is often assumed that a decision-maker assesses the desirability and likelihood of the possible outcomes of choice alternatives, albeit subjectively and possibly with bias or error, and integrates this information through some type of expectation-based calculus to arrive at a decision.

% In any organizational decision-making process, a decision-maker is required to arrive at a judgment of which course of action is `good' or `better' and which is `bad' or `worse' but this is rarely easy.  

% This assessment requires that the decision-maker determine what is \textit{valued}---attributes through which the desirability of different options is to be evaluated--and that the decision-maker has a way to use observations---drawn from historical data or the perspectives of experts with relevant experience---to evaluate each option along valued attributes and arrive at an evaluative conclusion. 

==> sections-old/01_introductionsv2.tex <==
% % Relevant Papers:

% % Multiple representations for ideas: https://arxiv.org/pdf/2308.03921.pdf

% % Multi-resolution representations for ideas:
% % https://arxiv.org/pdf/2306.09328.pdf

% % but focuses more on version control

% % Maybe: https://arxiv.org/pdf/2302.14165.pdf

% % Paul Resnick's paper on soliciting expert recommendations can help set up the problem:https://pubsonline.informs.org/doi/abs/10.1287/mnsc.1050.0379


% % Dourish paper ofcourse

% % Decision Analysis for Healthcare Managers (especially the MAV chapter)

% % Decision Synthesis

% In any 

% There is a great disconnect between the design of portable interactive electronics and the design of the energy storage systems
% that power them. Consider the following: Alice is a designer who
% wishes to create a small interactive electronic ring to wear for a
% few hours at an upcoming special event. She begins by prototyping on a benchtop, using a power supply to power her electronics
% and focusing on refning her desired interactions and aesthetic elements, which she can iteratively prototype quickly. Once satisfed,
% Alice makes the appropriate electrical measurements to estimate
% the power consumption of her system. The system turns out to be
% very low power, requiring only 1V and consuming at most 1mA.
% Looking through an online catalogue, Alice fnds that the smallest battery that can suit her needs is a 3.7V, 110mAh lithium ion
% battery that costs \$6 (USD) 1. It will arrive in 2-5 days. While the
% battery is relatively small – half the size of a thumb – it is still large
% for Alice’s on-fnger application and will power the system almost
% 100 times longer than necessary. Alice is further disappointed to
% realize that after the event, she will have no use for the battery,
% and it will simply sit in her drawer and gather dust alongside her
% growing collection of old batteries. While waiting for the battery
% to arrive, Alice adjusts her design, increasing its size substantially
% to accommodate, hide, and protect the battery.

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{images/discern-intro.pdf}
    \caption{}
    TODO update participant count, mentor count, add the fourth incubator, Add one feature during fourth incubator to be "Improved feedback visibility, Add interview w/ 1 entrepreneur in April 2023" 
    \label{fig:timeline}
\end{figure} 

Organizations are characterized by representative decision making: an individual decision maker is often tasked with evaluating and picking a course of action even if the decision concerns many. Because decision-making is centralized but information may be distributed, it may seem that a necessary limitation of this approach is that it risks excluding potentially useful information that may inform evaluation. Consider the case of a healthcare program manager responsible for deciding whether the hospital's budget for quality improvement projects is better spent pursuing improvements in the cardiac care unit or the respiratory care unit. They do not directly interact with the patients or work in the unit and so their understanding of the true state of affairs in either unit is limited. For this reason, CSCW research has long been interested in the creation of an ``information superhighway'': translating everything that can be captured into digital data and presenting these through dashboards so that decision-makers may observe relevant facts. In the previous example, historical data such as each unit's readmission rates, complication rates, utilization rates, or operating costs can inform an assessment of how each potential course of action is anticipated to fare along different criteria.

However, decisions for which distributed data might most help---where the decision-maker is removed from the context of the decision---are precisely those decisions whose impacts are distributed.

attention is limited and decisions concern people

However, to use available facts to pick the `best' course of action, a decision-maker must also make value judgments about what objective the decision ought to accomplish---which criteria should even be considered and the relative value placed on each. This involves reconciling the---often conflicting---preferences of individuals into a common objective. 

What results is a messy iterative process


This paper focuses on the deliberation inherent in many organizational decisions, asking if (and how) intelligent tools can support it. In doing so, we report on a series of design activities conducted with managers in a large tech company, reflecting on our activities, designed artifacts, how managers responded to our design choices, and the design opportunities they (and we) identified. Through formative surveys and interviews we examined managers' current practices of deliberative reasoning reflecting on what intelligent tools might support. Based on our findings, we developed \textbf{DISCERN}, an Excel extension. Finally, we conducted user enactments, asking four managers to enact a loosely scripted scenario they were familiar with---a simulation of a team meeting in which they are attempting to make decision---with and without our design concept---DISCERN. We used these enactments as boundary objects inviting managers to reflect on how DISCERN supported or complicated their needs, to observe underlying social boundaries, and to further identify opportunities for possible system designs.

==> sections-old/02_related.tex <==
\ed{\subsection{Meso-level Social Decision Making}}

\ed{Recent research in HCI has focused on understanding how to design data-driven support for social decision making. In domains ranging from criminal justice, urban planning, social work, content moderation, and administration, individual decision-makers are responsible for making decisions that rest on judgements about other individuals who are then subject to the decision. For instance, parole decisions involve making judgements about the defendent's likelihood of committing a crime in the future. Content moderators in an online community make judgements about the intentions of the author and potential harms to other members, in deciding whether to publish a given piece of content. Child maltreatment hotline workers make judgements about the risk a child faces in deciding whether a referral should be investigated further. Because they rest on inferences about intentions and beliefs of others, and because the impacts are felt by others, these decision-making tasks have been referred to as ``social decision-making'' in prior work.} 

\ed{In many of these domains, the data infrastructures already in use for formalization and rationalization---electronic management systems, surveys---and the computer-mediated nature of activities, generate a wealth of relevant data that can be brought to bear on decision-making efforts. Several research and commercial efforts have attempted to help decision-makers use available data to make case-specific evaluations through dashboards, data visualizations, and predictive models, in the hopes that data-driven decisions may help the decision-maker overcome their own biases and limitations to make ``better decisions'', improving either efficiency, equitability, explainability, or perceived legitimacy of the decisions. In addition to furthering our understanding of how technologies support or complicate decision-making in these domains, this line of work has also demonstrated how individuals faced with making social decisions confront needs and constraints not felt when making personal decisions. Most notably, whereas individuals decision-makers making personal decisions maybe unsure about what ought to be considered in the choice between alternatives, social decisions present the added challenge that even if individual stakeholders are certain about what they think ought to matter, there may be disagreement among stakeholders. In response, researchers have     }


\ed{By and large, HCI research studying the design and deployment of technological support in social decision-making has focused on decisions marked by a level of bureaucratic detachment and formalization such that the decision-maker is not expected to have a close ongoing relationship with those they are required to make judgements about. Indeed, in the domains described above, this separation is by design: it is intended to prevent decisions from being distorted by a concern with how they will affect one’s own reputation: the judge does not seek the social approval of the defendent. Many social decision-making scenarios, however, find expression somewhere in between the personal decisions an individual makes for themselves and social decisions with the level of bureaucratic separation typically studied---decisions where formalization is not entirely absent nor is very high, and where the decision-maker must make decisions that are binding on others but can not abandon concern for social approval and acceptance from the individuals for whom they are making decisions. Consider for instance,     }

\subsection{Defining ``decisions'' in organizational life and two frames for ``decision''-support in HCI}
Our work aims to understand and support decision-making practices in organizations. Before we can do so, however, it is useful to explicitly state what we mean by ``decisions''. In this paper, we use the definition of decisionsy extended by Alemi and Gustafson in their book `Decision Analysis for Healthcare Managers'~\cite{alemi2007decision} according to which a decision has the following five components:
``(1) multiple alternatives or options are available; (2) each alternative leads to a series of consequences; (3) the decision maker is uncertain about what might happen; (4) the decision maker has different preferences about outcomes associated with various consequences; (5) a decision involves choosing among uncertain outcomes with different values.'' We adhere to this definition not because it is the ``right'' definition but because the economic model of choice, encapsulated in the definition, features prominently in normative theories of organizational decision-making tracing back to Simon's seminal work~\cite{simon2013administrative}. It remains the benchmark in most teaching exercises on organizational decision-making~\cite{czarniawska2003forbidden, langley1989search}. Because it permeates teaching and prescription on decision-making as well as management books and training, many have shown that it affects organizational activities and managers' own interpretations of their actions~\cite{laroche1995decision, cabantous2010decision}. In a self-fulfilling way, because decision-making is taught this way, managers often think of their own work this way~\cite{laroche1995decision}. 

An attempt to define decisions this way also helps illustrate that decision-making can be challenging both when decision-makers are unsure about what values (criteria) they ought to consider in a decision (\textit{unclear values}) or when decision-makers are uncertain about how the options fare along criteria they value (\textit{uncertainty about future events}). These two ways to frame the challenge of decision-making often map to different (but complementary) lines of systems that have been extended as decision-support systems in HCI research. For group decision-making where conflicts in \textit{values} can present a primary impedance, a long line of systems have proposed affordances for conversational awareness~\cite{liu2018consensus, alonso2007visualizing, birnholtz2007exploratory, applegate1986group}, interventions~\cite{khadpe2022empathosphere, leshed2007feedback}, and communication workflows~\cite{zilouchian2015procid, kriplean2012supporting, farnham2000structured} to support value-focused conversations in groups that may allow them to mutually accept what values should be prioritized. On the other hand, tools aimed at individuals, where it is often \textit{uncertainty }and especially the capacity to analyze a large amount of information, that presents a primary impedance, another line of systems has considered how faceted search systems~\cite{hearst2006design, schraefel2006mspace, chang2019searchlens}, tools to visualize and explore tabular data~\cite{chimera1992value, spenke1996focus, liu2018consensus, chang2020mesh}, and automated summarization and predictive systems~\cite{yu2011aspect, li2010structure} can support decisions by lowering uncertainty along dimensions the decision-maker specifies. Our work draws on both these lines of work recognizing how decisions in organizations are neither ``purely'' group decisions nor ``purely'' individual. While these bodies of work establish the \textit{technical feasibility} of their approaches, we explore \textit{design opportunities} for the application of these techniques in the practice of organizational decision-making.

\subsection{Processes for considering stakeholder perspectives in organizational decision-making}

Representative decision-making---where a manager or leader is tasked with making decisions for a group---was developed as an approach for more rapid decision-making where pursuing large-scale consensus could be prohibitively time-consuming~\cite{crumley1995heterarchy, platt2022network}. This is why workplaces are often organized along the lines of control hierarchies~\cite{crumley1995heterarchy}. However, nothing about representative decision-making inherently changes the conditions under which a decision is considered good and acceptable by the group it is made for. Decision-making that is centralized may risk neglecting relevant information and perspectives that are distributed across the organization and in the minds of relevant stakeholders, which can compromise the perceived quality of outcomes (\textit{outcome favourability})~\cite{siegel2005moderating}. Further, people's attitude towards and acceptance of a decision depends not just on \textit{what} happens but also \textit{how} it happens~\cite{siegel2005moderating}: employees respond more positively when the procedures associated with the decision are viewed as fair (\textit{procedural fairness})~\cite{peterson1999can, folger1977distributive}. Representative decision-making can undermine perceptions of procedural fairness if it fails to consider the perspectives and preferences of impacted stakeholders. So, it should come as no surprise that even when individuals are authorized to make decisions they rarely exercise their authority in isolation. Managers consult their direct reports~\cite{lau2005importance, siegel2005moderating}. Maintainers of open-source software projects consult users~\cite{zilouchian2015procid, zilouchian2012consensus}. Healthcare managers consult healthcare professionals~\cite{wright2016evidence, alemi2007decision}. Deliberative practices through which managers consider stakeholders' preferences allow managers to access information~\cite{simon2013administrative, simon1957models}, understand individuals' preferences, and reconcile these into a common objective~\cite{gentry1982consensus}. It allows managers to understand and communicate the information and objectives that ought to be prioritized in a decision. 


However, inviting and managing participation has always been challenging. It can be challenging to structure conversations to effectively solicit inputs and to identify fundamental differences in preferences and reconcile them~\cite{benbunan2003comparative, keeney1996value}. Further, as conversations span different events and sources, it can become challenging to capture, organize, and understand the information that was gathered~\cite{courtney2001decision}. The magnitude of these intersecting challenges is most clearly evidenced by the existence of an entire professional body of experts---\textit{decision analysts}---often employed to help make complex organizational decisions~\cite{cabantous2010decision, howard1966decision, raiffa2002decision}. For the vast majority of decisions, where it may not be possible to consult a decision analyst, several decision-making frameworks~\cite{okoli2004delphi, keeney1996value} and elicitation techniques~\cite{o2005elicitation, hart2018training} have been proposed to aid managers in their deliberative decision-making practices.

Today, the diffusion of enterprise information technology promises to be a new solution to the myopia that representative decision-making entails, providing a new ``superhighway''~\cite{simon1988science} through which managers may understand the activities and work of others: through the information traces they leave. For instance, communication technologies and project management tools capture vast amounts of information about work activities as part of their regular operations~\cite{brynjolfsson2011strength, dormehl2015formula, lohr2015data}. This provides managers with an expansive view of the activities of their organization, creating an alternate pathway through which stakeholders' experiences may be considered in decision-making, in advance of actually talking to them. Contemporary trends towards more computer-mediated forms of work are only expected to increase the scope of what can be captured and observed through information traces~\cite{leonardi2018better, maltseva2020wearables}. At the same time, it creates new complications~\cite{dormehl2015formula}. Researchers have routinely pointed out that these ``superhighways'' only capture what we \textit{do} but not necessarily what we \textit{want}~\cite{seely2000social, dormehl2015formula} (e.g. just because an individual \textit{has} collaborated successfully with a particular team in the past, doesn't mean they \textit{want} to continue doing so). Within this evolving body of work, many have argued there remains a limited understanding of the concrete conditions under which decisions are actually made in organizations~\cite{cabantous2010decision, langley1995opening, laroche1995decision}. Therefore, in this moment, our work turns to the \textit{practitioners} of organizational decision-making, managers, asking: how do they \textit{practice} decision-making?

\subsection{Material used in organizational decision-making}
Decision-making is shaped not just by conceptual frameworks and facilitation strategies but also by the \textit{materials} used to enact decision-making processes~\cite{orlikowski2007sociomaterial, cabantous2010decision, dourish2017spreadsheets} (e.g. the whiteboard on which alternatives are listed, the slide deck around which discussion take place). Orlikowski suggests that organizational practices are not simply ``social'' or ``material'' but ``sociomaterial''~\cite{orlikowski2007sociomaterial}: social practice and digital materiality are tangled. That is, how we interpret and analyze information relies crucially on the interactive tools and representational systems we ``project''~\cite{cabantous2010decision} them into. Arguing how spreadsheets reconfigure organizational practice, Dourish says: ``when we think about spreadsheets not simply as repositories of data, but also as instruments of analysis, tools of engagement, and structures of participation and collaboration, then we see that these questions of granularity can be highly significant''~\cite{dourish2017spreadsheets}. It is by recognizing such entanglements that HCI research has attempted to contribute material environments for digital discourse~\cite{khadpe2022empathosphere, leshed2007feedback, applegate1986group} and digital data representation~\cite{kriplean2012supporting, zilouchian2015procid} as a way to influence decision-making practices. Building on this work, we investigate the material practices of managers when they make organizational decisions in an attempt to understand what is (not) supported by current materials and what parallel materials might support.

==> sections-old/discussions-old.tex <==
Our work aimed to understand managers' current practices of gathering, organizing, and analyzing information during decision-making and to identify opportunities for digital tools to support their practices. Our formative work revealed the challenges posed by fragmented information and the limited ways that these information spaces can be expressed or communicated. Further, our interviews revealed how managers did not want tools that obviate their face-to-face interactions with stakeholders but instead wanted representations to simply hold and reason about what they had heard. Based, on our findings we developed \sys{} which we used as a technology probe in our user enactment study. This further revealed how managers wanted tools that would allow them to ``qualculate'' and express objectives fuzzily to enable consensus. Below we interpret our findings to briefly mention opportunities and tensions for future research and practice attempting to develop decision-support tools for organizational use.

\subsection{Demonstrations of objectivity can clash with achieving consensus}
Across our formative work and user enactment, we found that managers' decision-making was ``qualculative'' and not purely calculative, both in private and in public. Even though instructional material, software tools, and professional decision analysts nudge decision-makers to model values and arrive at a ``score''~\cite{alemi2007decision}, managers in our studies felt this could threaten the achievement of consensus. Making decisions asocial through the precise quantification of the costs and benefits to each individual can shift the dynamic from communal sharing---where compromise is something that is shared---to equality matching---where individual compare their compromises to that of others~\cite{fiske1992four}. This raises questions about how the benefits of decision-support systems may be sensitive to the relationship between individuals involved in a decision-making situation, especially the relationship between the decision-maker and other stakeholders. Many systems proposed for consensus among groups may not account for the complexities of these real-world relationships as they are often tested among strangers brought together online or in an experiment~\cite{liu2018consensus, khadpe2022empathosphere}. There is an opportunity to investigate how these systems perform in smaller groups (that permeate many social institutions) where the maintenance of personal relationships is paramount. 

\subsection{Any imposition of structure can be undesirable in early stages}
Our formative studies found that managers did not always want to show their externalizations during conversations with stakeholders but instead wanted to begin with more abstract or minimal communication. When developing \sys{}, we had hoped that more abstract visual representations could serve this purpose. 
But our user enactments revealed how managers worked around \sys{}, often abandoning its representations, to fuzzily explicate their objectives so that they seem less final. One possible reason is that structure implies rigidity. Even though \sys{} provided ways to articulate structure visually and at different levels of abstraction, it still imposed rigidity. In the early stages when managers were still understanding the problem, they did not want to impose the structure on the group. This suggests opportunities for creating discourse platforms where structure can be invoked only when its need is felt. Further, tools can anticipate when decision-makers might want to transition to structured representations. Further, in early stages of a decision, groups might benefit less from structure and quantification and more from tools that support brainstorming. That is, decisions in early stages may be better represented as design problems~\cite{simon1996social}. 

\subsection{Tools that enable generative compromise.} \sys{}, and several tools for group decision-making, can reinforce a view of decision-making as a choice or an allocation between available alternatives. This framing precludes the development of new or alternate solutions. Many organizational decision-making processes however begin without a set of alternatives and may even conclude with just one bespoke ``solution''~\cite{mintzberg1976structure}. There is an opportunity, then, to explore how decision-making processes and tools can support \textit{generative compromise} through the design of collective decision representations and discourse affordances. By allowing individuals to propose and iterate on collective solutions, such tools could allow new, collectively intelligent solutions to emerge while also making people feel heard. Several tools have been proposed to address coordination challenges at large-scales~\cite{kriplean2012supporting, zhang2017wikum}, but these often focus on affordances that allow synthesis and summarization of proposals once generated. There remain opportunities to design representations and affordances that foster generativity by providing points for jumping off.

==> sections-old/ue-old.tex <==










In the next phase of our study, we conducted a series of user enactment sessions to understand how DISCERN -- a system designed to externalize multi-resolution representational structures -- supported or complicated their decision-making needs. 
We leverage user enactments~\cite{??} to simulate a real-world scenario where a manager gathers information and reconciles individual preferences toward achieving team-based decision-making. 
Within each manager participant, we also contrast the experience of using DISCERN with using a plain spreadsheet because our formative study found the use of spreadsheets to be common among managers. 



\jina{I'm thinking it's better to talk about the protocol before participants so they understand who's who}

\subsection{Study Protocol}

\jina{Not saying this is a counter-balanced or two-condition experiment because I want to tone down formality}
\jina{Need to be consistent about scoring system, rubric, decision rule, decision rubric?}
In a simulated user enactment scenario, a manager participant was debriefed as someone who works in a hypothetical multinational technology company called HeliCorp and leads a hypothetical team of four team members.
Based on a mandate by the organizational leaders, the manager was tasked with deciding (1) the remote workday of the week and (2) the designated quiet hours for the team.

Each interested manager participant was given a consent form to sign and an intake survey that optionally captured their demographics (e.g., age, gender, role, tenure, team size). 
Each interested team member participant was given a consent form to sign and an intake survey that captured their age, gender, and subjective assessments of similarity to eight team member personas. \jina{Also sharing in case it's helpful but probably appendix material} The personas provided are:
\begin{itemize}
    \item \textit{Alex}: Alex is a senior software engineer who's been with the company for five years. They live with their partner and their two young kids. They are highly motivated and productive and often take the lead on complex tasks. 
    \item \textit{Casey}: Casey is a mid-level developer who joined the company two years ago. They live alone and enjoy cycling and hiking during their free time.
    \item \textit{Jordan}: Jordan is a junior software engineer who's just finished their first year at the company. They live with their parents and two siblings and have a keen interest in video gaming. 
    \item \textit{Riley}: Riley is a highly skilled QA engineer who's been with the company for three years. They live with their partner and two dogs and love spending time in the park with their pets. 
    \item \textit{Taylor}: Taylor is a database engineer who's been with the company for two years. They live in a flatshare with three other people and play in a local band. 
    \item \textit{Morgan}: Morgan is a project manager who's been with the company for seven years. They live alone and enjoy reading and traveling in their free time. 
    \item \textit{Lee}: Lee is an experienced UI/UX designer who's been with the company for four years. They live with their spouse and cat, and they are deeply interested in art and design. 
    \item \textit{Charlie}: Charlie is a systems analyst who's been with the company for six years. They live with their partner and two children. They are highly respected for their skills and dedication. 
\end{itemize}

Each consented manager participated in two 1-hour sessions, and each consented team member participated in the second 1-hour session.
The first session involved managers coming up with a decision rubric to evaluate different courses of action in the two decision-making tasks mentioned above. 
The second session involved the user enactment where the manager discussed and deliberated on their decision rubric with four random participants who played the role of team members. 

For the first half of the first session, the manager was given a recorded tutorial on the DISCERN system and one of the two decision-making tasks in a random order. Before interacting with the system, we asked the manager to self-report on the perceived difficulty of the task and to ideate at least three relevant attributes for the decision-making task. The manager was then asked to use the DISCERN system to devise their decision rubric for about 12-13 minutes. After that, the manager was asked a series of post-task questions including the perceived difficulty of the task, ease of iteration on the rubric, satisfaction with the attributes, satisfaction with the rubric, perceived preparedness for a constructive meeting with the team, the extent to which the decision rubric changed during the task, and general feedback about the spreadsheet environment. For the second half of the first session, the manager was given a generic spreadsheet for the remaining decision-making task, and the procedure was identical to that of the first half.

\jina{Putting the following in just in case it's needed. Or we omit and put into appendix}
For each of the decision-making tasks, the manager participants were given the following instructions:

\paragraph{Which day of the week should be a remote workday?}
Your organization currently has a workplace policy for every worker to be fully on-site. However, recent research has indicated that allowing one remote day a week may improve worker focus and productivity. Based on this, your organizational leaders have mandated that each manager confer with their team and decide on one day of a work week to work remotely by the end of the day. In making this decision, organizational leaders have advised that managers choose one day of the week after comparing how cross-team collaboration, productivity patterns, personal commitments, and team morale might be affected based on the choice of the day. They have also advised that the decision be equitable so that no one team member is disproportionately disadvantaged. However, they have left it up to your judgment to decide the extent to which these factors should affect the decision and to evaluate different days along these factors and make a final decision.  
You know that most social events happen on Thursday and Friday so enforcing that your team works from home on those days could dampen team morale. Given your limited visibility into the team members' work routines, you have set up a meeting to invite input from different members to evaluate other factors for each day. For instance, for a given day you might ask each member whether they collaborate in-person with other teams on that day to evaluate the number of people whose cross-team collaborations would suffer if asked to work from home on that day. 
Your options are Monday, Tuesday, Wednesday, Thursday, Friday.

\paragraph{Which hours of the day should be quiet hours?}
Your organization, in an attempt to bolster productivity and promote a culture of focus, is considering the implementation of a daily "quiet hour" policy. This would involve a set 2-hour block of time each day during which employees are encouraged to concentrate on their work with minimal interruptions. Your organizational leaders have tasked each manager with discussing this with their teams and deciding on the quiet hours of the day by the end of the day. While deciding this, managers have been advised to consider the personal productivity rhythms, external collaboration patterns, and disruption to existing routines. They have also stressed that this decision should be fair and should not unfairly disadvantage any team members. The actual weight of these factors and how they are assessed in the final decision, however, is left up to your judgment. 
It's important to note that the timing of these quiet hours could potentially interfere with regular work habits, collaborative meetings, or even personal commitments. Moreover, it's a well-known fact in your organization that the after-lunch hours are usually more social and team bonding oriented, so declaring those as quiet hours might impact the team culture adversely. Since you don't have a complete understanding of everyone's daily work routines, you have decided to arrange a meeting to gain insight from the team to make a well-rounded decision. For example, you might ask each team member about their peak productivity hours or when they usually schedule their collaborative meetings. 
Your options are 9-11 am, 10-12 am, 11am-1pm, 1-3pm, 2-4pm, and 3-5pm.

\jina{I forget, was it always DISCERN first?}
For the second session, the manager was asked to use their decision rubric to engage in a discussion with the four team members and incorporate their input to arrive at a final decision for each task. 
Each of the four team members assigned to this manager was given one of the eight personas that best matched their subjective assessments of similarity during their intake and was given instructions about how to role-play that persona during the discussion.
In addition to the persona description given during intake, the instructions included each persona's preference for the remote workday and quiet hours as well as a detailed list of rationale for their preferences. For example, Morgan's persona included Tuesday as the preference for the remote workday with the following description: ``As a project manager, my role demands a balance of team interaction and strategic planning. While Mondays are about syncing with the team, Tuesdays are my sanctuary for strategic thinking and mapping out the week. Working remotely then aids my focus, dovetailing beautifully with my love for reading and traveling. Whether it's catching up on a new book, attending a travel expo, or simply enjoying the tranquillity of my home, a remote Tuesday ensures I get the best of both my professional and personal worlds.'' 


At the beginning of the session, we welcomed the manager participants and four team member participants and described how the session would proceed. 
During the first half of the second session, the manager drove the discussion of their first decision-making task using DISCERN with their hypothetical team of four employees for approximately 15 minutes. After the discussion, we pulled the manager into a breakout room to ask for their final decision, a short explanation email about the decision, and subjective ratings for the effectiveness of the meeting in their decision-making, their satisfaction with the final decision, their satisfaction with the email explanation, and to what extent they felt their understanding of decision changed or they were able to adapt during the meeting.
Then the manager proceeded back to the main room and followed the same procedure for their second decision-making task using the spreadsheet with the same four team members playing the same personas.
At the end of both discussions, team member participants were asked to leave the session. 
Then we proceeded to debrief the experience with the manager participant focusing on comparing their experiences between DISCERN and spreadsheet alone. We asked if they found DISCERN to be more or less helpful in reflecting and iterating on the decision rubric, documenting the decision rubric, communicating the decision rubric, guiding the discussion with the team, arriving at a consensus within the team, gaining confidence in the decision rubric, gaining confidence in the final decision, and capturing and communicating the decision rationale. We also asked for examples of how DISCERN was more or less helpful, whether they would recommend the system to others, or any other comments or suggestions.

Each manager participant was compensated with a \$75 gift card, and each team member participant was compensated with a \$25 gift card. Our interview study protocol was approved by the lead institution's Institutional Review Board (IRB).


\subsection{Participants}

We recruited four managers, two of whom were repeat participants from our interview study. \jina{How important is the manager demographics. 2 answered. The other 2 are OOF}
